Simulation-based optimal Bayesian experimental design for nonlinear systems

The optimal selection of experimental conditions is essential to maximizing the value of data for inference and prediction, particularly in situations where experiments are time-consuming and expensive to conduct. We propose a general mathematical framework and an algorithmic approach for optimal experimental design with nonlinear simulation-based models; in particular, we focus on finding sets of experiments that provide the most information about targeted sets of parameters. Our framework employs a Bayesian statistical setting, which provides a foundation for inference from noisy, indirect, and incomplete data, and a natural mechanism for incorporating heterogeneous sources of information. An objective function is constructed from information theoretic measures, reflecting expected information gain from proposed combinations of experiments. Polynomial chaos approximations and a two-stage Monte Carlo sampling method are used to evaluate the expected information gain. Stochastic approximation algorithms are then used to make optimization feasible in computationally intensive and high-dimensional settings. These algorithms are demonstrated on model problems and on nonlinear parameter estimation problems arising in detailed combustion kinetics.

==> Makefile <==
all: main.pdf

dvi: main.dvi

main.pdf: LatexPDF
	pdflatex --shell-escape -output-format pdf main.tex
	bibtex main
	pdflatex --shell-escape -output-format pdf main.tex
	pdflatex --shell-escape -output-format pdf main.tex

main.dvi: LatexDVI
	latex main.tex
	latex main.tex
	bibtex main
	latex main
	latex_count=5 ; \
	while egrep -s 'Rerun' main.log && [ $$latex_count -gt 0 ] ;\
	    do \
	      echo "Rerunning latex...." ;\
	      latex main.tex ;\
	      latex_count=`expr $$latex_count - 1` ;\
	    done

clean:
	rm -f *.bbl *.blg *.ps *.dvi *.aux *.toc \
	      *.idx *.ind *.ilg *.log *.out *.spl *.brf

LatexDVI:
	echo "Running latex..."

LatexPDF:
	echo "Running pdflatex..."


==> polynomialChaos.tex <==
\subsection{Polynomial chaos}
\label{ss:polynomialChaos}

Focus mainly on the NISP formulation. Discuss sparse quadrature and
DASQ (toy problems?), but detailed comparisons to other integration
methods not needed (perhaps just have a couple of paragraphs
discussing other options).

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.6\textwidth]{figures/polynomialChaos/sparseSimplex}
  \caption{This is a figure.}
  \label{f:simpleModel}
\end{figure}

\begin{figure}[htb]
  \centering
  \subfigure[Stuff a]
  {
    \includegraphics[width=0.47\textwidth]{figures/polynomialChaos/CCD2Tensor}
%    \label{f:typicalTProfile}
  }
  \subfigure[Stuff b]
  {
    \includegraphics[width=0.47\textwidth]{figures/polynomialChaos/CCD2L5}
%    \label{f:typicalXProfile}
  }
  \subfigure[Stuff c]
  {
    \includegraphics[width=0.47\textwidth]{figures/epsHolder}
%    \label{f:typicalXProfile}
  }
  \caption{Grids!}
%  \label{f:typicalProfiles}
\end{figure}


